A Unified Discretization Approach to Compute-Forward: From Discrete to Continuous Inputs

Compute-forward is a coding technique that enables receiver(s) in a network to directly decode one or more linear combinations of the transmitted codewords. Initial efforts focused on Gaussian channels and derived achievable rate regions via nested lattice codes and single-user (lattice) decoding as well as sequential (lattice) decoding. Recently, these results have been generalized to discrete memoryless channels via nested linear codes and joint typicality coding, culminating in a simultaneous-decoding rate region for recovering one or more linear combinations from $K$ users. Using a discretization approach, this paper translates this result into a simultaneous-decoding rate region for a wide class of continuous memoryless channels, including the important special case of Gaussian channels. Additionally, this paper derives a single, unified expression for both discrete and continuous rate regions via an algebraic generalization of R\'enyi's information dimension.

==> figs/introduction.tex <==
\begin{tikzpicture}[start chain]
	\matrix[matrix of nodes, nodes={draw, anchor=center}, on chain] (chain-1) {
		|[name=enc1, minimum height=8mm]| {encoder~1} \\[8mm]
		|[name=enc2, minimum height=8mm]| {encoder~2} \\
	};
	\node[on chain, draw, minimum height=8mm] (channel) {$P_{Y^n|X_1^n,\dotsc,X_K^n}$};
	\node[on chain, draw, minimum height=8mm] (decoder) {decoder};
	\draw[<-] (enc1.west) --+ (-5mm,0) node[left] {$M_1$};
	\draw[<-] (enc2.west) --+ (-5mm,0) node[left] {$M_K$};
	\draw[->] (enc1.east) --+ (3mm,0) node[right, anchor=west] {$X_1^n \in \mathbb{F}_\q^n$} -- ($(channel.north west)!.2!(channel.south west)+(-3mm,0)$) -- ($(channel.north west)!.2!(channel.south west)$);
	\draw[->] (enc2.east) --+ (3mm,0) node[right, anchor=west] {$X_K^n \in \mathbb{F}_\q^n$} -- ($(channel.north west)!.8!(channel.south west)+(-3mm,0)$) -- ($(channel.north west)!.8!(channel.south west)$);
	\draw[->] (channel.east) -- node[above] {$Y^n$} (decoder.west);
	\draw[->] (decoder.east) --+ (5mm,0) node[right] {$\hat{W}^n$};
\end{tikzpicture}

